Reinforcement Learning with Fast and Forgetful Memory

Nearly all real world tasks are inherently partially observable, necessitating the use of memory in Reinforcement Learning (RL). Most model-free approaches summarize the trajectory into a latent Markov state using memory models borrowed from Supervised Learning (SL), even though RL tends to exhibit different training and efficiency characteristics. Addressing this discrepancy, we introduce Fast and Forgetful Memory, an algorithm-agnostic memory model designed specifically for RL. Our approach constrains the model search space via strong structural priors inspired by computational psychology. It is a drop-in replacement for recurrent neural networks (RNNs) in recurrent RL algorithms, achieving greater reward than RNNs across various recurrent benchmarks and algorithms without changing any hyperparameters. Moreover, Fast and Forgetful Memory exhibits training speeds two orders of magnitude faster than RNNs, attributed to its logarithmic time and linear space complexity. Our implementation is available at https://github.com/proroklab/ffm.

==> conv_theorem.tex <==
\begin{theorem}
    Each dimension of FFM can represent a convolution of the input signal $o(t)$ with any filter $h(t)$, represented with arbitrary precision.
\end{theorem}

\begin{proof}
    From Equation \ref{eq:sn_single_dim}, we can represent a single dimension of FFM as:

    \begin{align}
    S &= \int_0^{\infty} x(t) \exp{(-t (\alpha + i\omega))} \, dt.
    \end{align}

    Then, the output of FFM can be described by Equation \ref{eq:output_gate}:

    \begin{align}
        y &= \mathrm{LN}(\ell_4(h || \ell_3(\mathrm{Flatten} (\Re{[S]} \mid\mid \Im{[S]}))) \odot \sigma(\ell_5( \bar{o}))
    \end{align}

    As we wish to prove a \textit{special case} of FFM, we can make some assumptions to simplify this equation. Let us assume that the sparsity-inducing term is non-active $\sigma(\ell_5( \bar{\bm{x}}_{k:n})) = 1$, the coefficients of $\ell_4$ corresponding to $h$ are $0$, and the coefficients corresponding to the real and imaginary parts of $z$ are equal. 
    
    Furthermore, since the dimension of the hidden state $x(t) \in \mathbb{R}^m$ is greater than the dimension of the $o(t) \in \mathbb{R}^d$, the same dimension of $o(t)$ can map to multiple dimensions in $x(t)$. Let us assume that that $\mathcal(D)(i)$ is a set of dimensions in $x(t)$ which are copies of dimension $i$ of $o(t)$ (\textit{i.e.} there is sparsity in the mapping $\ell_1$). Then, for dimension $i$ of $o(t)$, the output can be represented as:

    \begin{align}
        y_i = \sum_{j \in \mathcal{D_i}} c_j S_j 
    \end{align}

    where $c_j$ are coefficients from $\ell_3$ and $\ell_4$, and $S_j$ are the dimensions of of $S$ corresponding to dimension $i$ of $o(t)$.

    Putting these equations together, we obtain the output as a function of the observation $o(t)$ for a special case of FFM:

    \begin{align}
        y_i = \sum_{j \in \mathcal{D_i}} c_j \int_0^{\infty} o_i(t) \exp{(-t (\alpha_j + i\omega_j))} \, dt.
    \end{align}

    Rearranging this equation, we get:

    \begin{align}
        y_i = \int_0^{\infty} o_i(t) \cdot \sum_{j \in \mathcal{D_i}} c_j \exp{(-t (\alpha_j + i\omega_j))} \, dt.
    \end{align}
\end{proof}

==> tikz/modes.tex <==

\begin{tikzpicture}

\begin{groupplot}[
    group style={
        % set how the plots should be organized
        group size=4 by 3,
        % only show ticklabels and axis labels on the bottom
        x descriptions at=edge bottom,
        xticklabels at=edge bottom,
        yticklabels at=edge left,
        %x tick labels at=edge bottom,
        % set the `vertical sep' to zero
        %vertical sep=4pt,
        horizontal sep=1em,
    },
    height=8em,
    width=10em,
    ytick={-1, 0, 1},
    yticklabels={$-x_{j}$, $0$, $x_{j}$},
    ymax=1,
    ymin=-1,
    xmin=0,
    xmax=1024,
    samples=1000,
    domain=0:1024,
    xlabel=$t - j$,
    axis x line*=bottom,
    axis y line*=left,
    %x tick label style={/pgf/number format/sci},
    xtick={0, 500, 1e3},
    xticklabels={0, 500, 1e3}
    % set the x axis default to logarithmic
]
    \nextgroupplot[
        title=Timeless,
    ]
        \addplot[red] {1};
    \nextgroupplot[
        title=Lifelong,
    ]
        \addplot[red] {cos(deg(x/128))};
    \nextgroupplot[
        title=Long Term
    ]
        \addplot[red] {cos(deg(x/64))};
    \nextgroupplot[
        title=Short Term
    ]
        \addplot[red] {cos(deg(x/10))};
        
    \nextgroupplot[]
        \addplot[blue] {1};  
    \nextgroupplot[]
        \addplot[blue] {e^(0*x)};
    \nextgroupplot[]
        \addplot[blue] {e^(-0.002*x)};
    \nextgroupplot[]
        \addplot[blue] {e^(-0.02*x)};

    \nextgroupplot[
    ]
        \addplot[purple] {1};
    \nextgroupplot[
    ]
        \addplot[purple] {cos(deg(x/128)) * 1};
    \nextgroupplot[
    ]
        \addplot[purple] {e^(-0.002*x) * cos(deg(x/64))};
    \nextgroupplot[
    ]
        \addplot[purple] {e^(-0.02*x) * cos(deg(x/10))};
        
\end{groupplot}
\end{tikzpicture}
